Concept-aware Training Improves In-context Learning Ability of Language Models

Many recent language models (LMs) of Transformers family exhibit so-called in-context learning (ICL) ability, manifested in the LMs' ability to modulate their function by a task described in a natural language input. Previous work curating these models assumes that ICL emerges from vast over-parametrization or the scale of multi-task training. However, a complementary branch of recent theoretical work attributes ICL emergence to specific properties of training data and creates functional in-context learners in small-scale, synthetic settings. Inspired by recent findings on data properties driving the emergence of ICL, we propose a method to create LMs able to better utilize the in-context information, by constructing training scenarios where it is beneficial for the LM to capture the analogical reasoning concepts. We measure that data sampling of Concept-aware Training (CoAT) consistently improves models' reasoning ability. As a result, the in-context learners trained with CoAT on only two datasets of a single (QA) task perform comparably to larger models trained on 1600+ tasks.

==> old_texts.tex <==
% An important practical advantage of the few-shot approach is that the few shot models are able to perform in-context learning of a reasonable accuracy with much lower amounts of parameters;. For instance, the MetaICL of \citet{meta-icl} reaches a quality comparable to a 175-billion-parameter GPT-3 with only a 774-million-parameter model, by training the model explicitly in the format of the few-shot in-context learning.

% However, regardless of largely encouraging initial results in few-shot evaluations, both very large and smaller few-shot models expose some surprising and questionable behavioural artifacts. \citet{liu-etal-2022-makes} show that the ordering of demonstrations might have a significant impact on prediction quality in the few-shot settings. Similarly, \citet{lu-etal-2022-fantastically,TODO_ADD_MORE} find surprising sensitivity of in-context learners to the specific wording of the prompts. Finally, \cite{what-makes-incontext-work} show that the decay of the model performance when randomly permuting the contents of the demonstrations while keeping their labels harms the performance of few-shot minimally.

% These observations pose into question the \textit{depth} of understanding tasks by in-context learners. While it seems unlikely that stochastic models would capture a new task in a depth of a qualified human reader, it remains unclear how much performance gains of few-shot learning could be attributed merely to capturing surface-level associations such as non-trivial word collocations. Note that in few-shot settings, such associations might be much more difficult for a human annotator to uncover.

% A complementary feature of in-context learners' evaluation that yet remains uncontrolled concerns the representative selection of unseen evaluation tasks. 
% % We expect that the in-context learner will attain an ability of learning new tasks in a general training objective, such as Causal Language modeling \cite{Radford2018gpt} of GPT-3 or BLOOM, or answer generation conditioned by a massive mixture of tasks and prompts, in the case of T0 \cite{t0}. 
% The types of training tasks might condition the performance of in-context learners on unseen tasks; 
% A model that has seen many sequence classification tasks in its training mixture might perform better in new tasks of the type or similar type. 
% Similar might hold for the \textit{domains} of texts among the tasks; 
% consider a case of in-context learner trained for question answering (QA) on news texts and evaluated on a \textit{new} task of entity recognition of personal names and locations. 
% As such entities largely occur in the training QA dataset, an adaptation to such evaluation task of an unseen type, would be much easier than an identification of phone numbers, or other under-represented sensitive information.

% Our work aims to enhance our understanding in the two directions: 
% \begin{enumerate}
%     \item To assess in-context few-shot learners' ability to \textit{utilize} specific non-trivial \textit{concepts} exploited by the in-context demonstrations while disentangling such ability from capturing a \textit{task distribution} features, that are irrelevant for demonstrations' input-output mappings.
%     \item To assess and recommend features that can be used to choose the evaluation task for in-context learners \textit{representative} of the tasks' complexity given a fixed set of training tasks.
% \end{enumerate}

\section{Random Notes}
Motivation mentions
- Ability to 'learn in context' can not be demonstrated even by humans in non-informative contexts
- Evaluation in non-informative settings disproportionally rewards systems' ability to modulate based on inputs' distribution
- Achieving such property requires memorization that is possible only for the large-capacity models
- However, a scaling in this direction is not sustainable


- Hard demonstrations' selection can be too easy -- how do we make sure that few-shots do not exploit easier artefact than the shared concept?


\section{Problem Formulation}

* Mainstream formulation extending zero-shot to few-shot settings

\textbf{Zero-shot Learning}

\textbf{Few-shot Learning}


\subsection{Other Formulations}

\section{In-context Learning and Other Low-resource Methods}

* What are the other approaches to training models in low-resource settings?

* How does in-context learning differ from these?

\section{Previous Work on In-context Learning}

\subsection{Evaluation}

\section{Implications}

\begin{itemize}
    
    \item exploiting label semantics helps models adapt \cite{pet,lm-bff}
    \vfill
    
    \item small in-context few-shot models beat large  unsupervised models (on unseen tasks) \cite{t0, natural-instructions-2}
    \vfill
    
    \item few-shot performs better than zero-shot \cite{flan, natural-instructions-2}
    \vfill
    
    \item more of diverse pre-training tasks make better models (both zero-shot and few-shot) \cite{natural-instructions-2, natural-instructions-1, flan, t0}
    \vfill
    
    \item larger models work better \cite{flan, natural-instructions-2}
    \vfill
    
    \item current models don't learn much from the mapping between demonstrations and their labels \cite{what-makes-incontext-work}
    \vfill
    
    \item there are experiments about negative demonstrations, explanations, chain-of-thought reasoning, noisy-channel decoding, ... \cite{natural-instructions-1, natural-instructions-2, learn-from-explanations, noisy-channel}
    
\end{itemize}

\section{Open Questions}

* Insensitivity to few-shot labels


